Plagiarism Detection in Polyphonic Music using Monaural Signal Separation

Given the large number of new musical tracks released each year, automated approaches to plagiarism detection are essential to help us track potential violations of copyright. Most current approaches to plagiarism detection are based on musical similarity measures, which typically ignore the issue of polyphony in music. We present a novel feature space for audio derived from compositional modelling techniques, commonly used in signal separation, that provides a mechanism to account for polyphony without incurring an inordinate amount of computational overhead. We employ this feature representation in conjunction with traditional audio feature representations in a classification framework which uses an ensemble of distance features to characterize pairs of songs as being plagiarized or not. Our experiments on a database of about 3000 musical track pairs show that the new feature space characterization produces significant improvements over standard baselines.

==> dtw.tex <==
\section{Joint Feature Set Using DTW}
Dynamic time warping (DTW) is an efficient algorithm for handling the matching of non-linearly expanded or contracted signals \cite{Sakoe1978}. The optimal alignment between the two sequences is efficiently calculated using dynamic programming.

Given two time sequences $X=\langle x_1, x_2, ..., x_m \rangle$ and $Y=\langle y_1, y_2, ..., y_n \rangle$, it fills an $m$-by-$n$ matrix representing the distances of the best possible partial path using:
\begin{equation}
D(i,j) = min(D(i,j-1),D(i-1,j),D(i-1,j-1))+d(i,j)
\end{equation}
where $1\leq i\leq m, 1\leq j\leq n, d(i,j)$ represents the distance between $x_i$ and $y_j$, and $D(1,1)$ is initialized to $d(1,1)$.

When a music piece copies another musical piece without proper acknowledgement, even a matching portion of only 2-3 seconds might be treated as a case of plagiarism. Computing a degree of resemblance using the DTW to identify all possible cases of plagiarism is a non-trivial problem. In past cases of musical plagiarism, we observed that, almost in all cases, the two musical pieces differed in rhythm, while retaining some other musical property.

Thus for the rhythm-based features, we use a modified version of the DTW \cite{Muller2009}. We use local weights to prefer an insertion or deletion, to a substitution to better account for the variation in rhythm. The modification is of the form,
\begin{equation}
D(i,j) = min \begin{cases}
  D(i-1,j-1)+w_d.d(i,j) \\
  D(i,j-1)+w_h.d(i,j) \\
  D(i-1,j)+w_v.d(i,j)
\end{cases}
\end{equation}
We keep $w_d$ much larger with respect to $w_h$ and $w_v$. This follows from the fact that, even though the DTW would effectively match two sequences having the same musical property with varying rhythm, the distance between the two sequences would still be large owing to the numerous insertions and deletions required for matching the two time-varying sequences. This would not be representative of the similarity observed between the sequences. Thus, using a lower weight for insertion and deletion would help in bringing out this similarity.

Intuitively, however, a disadvantage of this modification would be that the warping path might get stuck in some position due to a local acceleration or deceleration by a large factor. This is overcome by constraining the slope of the warping path. This ensures that there exists a path between the two sequences if and only if their lengths differ at most by a factor of the upper bound of the allowed slope.



==> notes_comparisonWithExistingSystem_bak.tex <==
\subsubsection{Comparison With Existing Systems}

Instances of our method were tested with some existing systems in the detection of near-duplicate music documents. Some of the recent work done in this regard involve the works of Hanna et. al. \cite{Hanna2011} and Robine et. al. \cite{Robine2007}.

The difficulty in the detection of musical plagiarism compared to systems based on the detection of near-duplicate music documents are that, in the latter case, the music pieces, in general are of very similar notes. This is in sharp contrast to many plagiarism cases, where sequences made of very different notes can be musically very similar. Moreover, plagiarised copies may have a very small sequence similar to the original song, while systems which detect near-duplicate music documents consider (and function with) only longer sequences of similarity.

Both the systems achieved good success in detecting successful plagiarism cases using monophonic melody sequences. However, both systems had very limited success for polyphonic melody sequences even for plagiarism cases containing a high level of similarity, such as the Bright Tunes Music v. Harrisongs Music case involving the songs He's So Fine and My Sweet Lord. In contrast, our method was successful in detecting plagiarism for the songs in question.

In another plagiarism suit between Palmieri v. Estefan, the defending song `Oye Mi Canto' had only a 2 second clip similar to `Paginas De Mujer' in the chorus. Though the judge however ruled against the plaintif	f due to their inability to prove that the defendant had access to the plaintiff's work, the two songs were substantially similar. Our method was successful in detecting original copies of these two songs as plagiarised copies, showing a significantly better margin for the length by which the two songs need to be similar for successful detection. %This shows our method is able to identify songs having a small part similar compared to the full song.

Our method, however, failed to detect similarity in some cases where the copied portion was made very faint and in the background. An example would be the similarity in a guitar riff in the musical pieces involved in the La Cienega Music Co. v. ZZ Top plagiarism suit.
